Characterizing Developer Use of Automatically Generated Patches

We present a study that characterizes the way developers use automatically generated patches when fixing software defects. Our study tasked two groups of developers with repairing defects in C programs. Both groups were provided with the defective line of code. One was also provided with five automatically generated and validated patches, all of which modified the defective line of code, and one of which was correct. Contrary to our initial expectations, the group with access to the generated patches did not produce more correct patches and did not produce patches in less time. We characterize the main behaviors observed in experimental subjects: a focus on understanding the defect and the relationship of the patches to the original source code. Based on this characterization, we highlight various potentially productive directions for future developer-centric automatic patch generation systems.

==> figures/c_cpp_experience.tex <==
\begin{tabular}{lrr}
\toprule
Experience Level &  C &  C++ \\
\midrule
   No experience &  1 &    2 \\
  Several months &  1 &    0 \\
          1 year &  3 &    2 \\
         2 years &  2 &    3 \\
         3 years &  3 &    2 \\
         4 years &  1 &    0 \\
         5 years &  1 &    3 \\
\bottomrule
\end{tabular}


==> figures/correct_solutions_details.tex <==
\begin{tabular}{lllll}
\toprule
 Study &     Treatment &  Subject &      Bug &  Time / Alloted (min.) \\
\midrule
  Long &       Control &     5 &  libtiff &           18 / 40 \\
  Long &       Control &    13 &      php &           14 / 40 \\
  Long &  Experimental &     2 &  libtiff &           36 / 40 \\
  Long &  Experimental &     3 &      php &           21 / 40 \\
 Short &  Experimental &     9 &  libtiff &           24 / 25 \\
\bottomrule
\end{tabular}


==> figures/mean_submission_times.tex <==
\begin{tabular}{llrr}
\toprule
Experiment Length &         Group &  Mean (minutes) & sd \\
\midrule
             Long &       Control &           26.38 & 11.92 \\
             Long &  Experimental &           25.71 & 13.44 \\
            Short &       Control &           22.50 &  2.89 \\
            Short &  Experimental &           17.93 &  4.45 \\
\bottomrule
\end{tabular}

